Back2Future: Leveraging Backfill Dynamics for Improving Real-time Predictions in Future

In real-time forecasting in public health, data collection is a non-trivial and demanding task. Often after initially released, it undergoes several revisions later (maybe due to human or technical constraints) - as a result, it may take weeks until the data reaches to a stable value. This so-called 'backfill' phenomenon and its effect on model performance has been barely studied in the prior literature. In this paper, we introduce the multi-variate backfill problem using COVID-19 as the motivating example. We construct a detailed dataset composed of relevant signals over the past year of the pandemic. We then systematically characterize several patterns in backfill dynamics and leverage our observations for formulating a novel problem and neural framework Back2Future that aims to refines a given model's predictions in real-time. Our extensive experiments demonstrate that our method refines the performance of top models for COVID-19 forecasting, in contrast to non-trivial baselines, yielding 18% improvement over baselines, enabling us obtain a new SOTA performance. In addition, we show that our model improves model evaluation too; hence policy-makers can better understand the true accuracy of forecasting models in real-time.

==> Tables/accuracy2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{wraptable}{l}{.6\linewidth}
\centering
\vspace{-0.2in}
\caption{\model consistently refines all models. \% improvements in MAE and MAPE scores averaged over all 50 regions from May 2020 to Dec 2020.}
\label{tab:mainresult}
\scalebox{0.8}{
\begin{tabular}{l|l|l|l|l|l}
                          &                         & \multicolumn{2}{l|}{\textbf{k=2}} & \multicolumn{2}{l|}{\textbf{k=4}} \\ \hline
\textbf{Cand. Model}      & \textbf{Refining Model} & MAE             & MAPE            & MAE             & MAPE            \\ \hline
\multirow{5}{*}{Ensemble} & \ffnreg            & -0.35           & -0.12           & 0.81            & 0.36            \\ \cline{2-6} 
                          & \modelreg            & -2.23           & -1.57           & -1.13           & -2.36           \\ \cline{2-6} 
                          & \bseqregt           & -1.45           & -2.73           & -5.2            & -4.78           \\ \cline{2-6} 
                          & \bseqreg          & 1.42            & 0.37            & 0.72            & 0.28            \\ \cline{2-6} 
                          & \model             & \textbf{5.18}   & \textbf{5.47}   & \textbf{3.61}   & \textbf{6.3}    \\ \hline
\multirow{5}{*}{GT-DC}    & \ffnreg            & -2.42           & -1.51           & -1.86           & -0.49           \\ \cline{2-6} 
                          & \modelreg            & -3.02           & -3.41           & -2.81           & -3.26           \\ \cline{2-6} 
                          & \bseqregt           & 2.24            & 3.51            & 1.6             & 0.57            \\ \cline{2-6} 
                          & \bseqreg          & 2.13            & 3.84            & 1.42            & 2.27            \\ \cline{2-6} 
                          & \model             & \textbf{12.68}  & \textbf{12.59}  & \textbf{9.64}   & \textbf{8.97}   \\ \hline
\multirow{5}{*}{YYG}      & \ffnreg            & -2.08           & -1.34           & -1.37           & -3.06           \\ \cline{2-6} 
                          & \modelreg            & -3.84           & -6.99           & -9.29           & -5.81           \\ \cline{2-6} 
                          & \bseqregt           & -1.25           & -0.7            & -6.65           & -5.45           \\ \cline{2-6} 
                          & \bseqreg          & -1.78           & -2.26           & -0.61           & -0.43           \\ \cline{2-6} 
                          & \model             & \textbf{8.84}   & \textbf{5.98}   & \textbf{6.8}    & \textbf{5.27}   \\ \hline
\multirow{5}{*}{Umass-MB} & \ffnreg            & -3.25           & -5.74           & -1.44           & -4.84           \\ \cline{2-6} 
                          & \modelreg            & -8.2            & -7.54           & -5.99           & -7.43           \\ \cline{2-6} 
                          & \bseqregt           & -2.16           & -1.88           & -2.29           & -2.31           \\ \cline{2-6} 
                          & \bseqreg          & 1.58            & 0.86            & 0.06            & 0.03            \\ \cline{2-6} 
                          & \model             & \textbf{5.21}   & \textbf{4.92}   & \textbf{3.94}   & \textbf{3.49}   \\ \hline
\multirow{5}{*}{CMU-TS}   & \ffnreg            & -5.24           & -4.93           & -3.19           & -6.7            \\ \cline{2-6} 
                          & \modelreg            & -8.17           & -8.21           & -3.75           & -9.1            \\ \cline{2-6} 
                          & \bseqregt           & -0.67           & -0.57           & -0.38           & -0.12           \\ \cline{2-6} 
                          & \bseqreg          & 1.46            & 1.05            & 2.11            & 2.84            \\ \cline{2-6} 
                          & \model             & \textbf{8.75}   & \textbf{10.48}  & \textbf{6.93}   & \textbf{6.28}   \\ \hline
\end{tabular}
}
\vspace{-0.1in}
\end{wraptable}

==> backfill_prob.tex <==
\section{Setup}

%Here we provide the mathematical definitions and notations to describe backfill as a problem for real time forecasting. 
Here we give the background, notation and definitions to set up backfill in real-time forecasting. 
In addition, it is important to note that the data in backfill is the same used for real-time forecasting, but seen from a different perspective.

% first attempt alex
% \aditya{I do not understand the 'real-time sequence'. is $D^t$ for a particular 't' the sequence? How can one timestamped dataset be a sequence. We need to say what is Xt and Yt, maybe Xti is a time-series from [1..t] something like that}
\par\noindent\textbf{Real-time forecasting.} 
At prediction week $t$, $x^{(t)}_{i,1:t}$ is a time series from 1 to $t$ for feature $i$\footnote{In practice, we have some features that incur in delays; that means that, at time $t$, we have data until t-$\delta$. This has been taken care of in our analysis and can be incorporated to our notation, as we show in our supplement.}, and the set of all features results in the multi-variate time series $\mathcal{X}^{(t)}_{1:t}$.
Similarly, $\mathcal{Y}^{(t)}_{1:t}$ is the forecasting target(s) time series.
Further, let's call all data available at time $t$, $\mathcal{D}^{(t)}_{1:t} = \{ \mathcal{X}^{(t)}_{1:t},  \mathcal{Y}^{(t)}_{1:t} \}$ as \emph{\underline{real-time sequence}}. 
%to our data available at time $t$ and denote it as $\mathcal{D}^{(t)}_{1:t} = \{ \mathcal{X}^{(t)}_{1:t}, \mathcal{Y}^{(t)}_{1:t} \}$. 
For clarity we refer to `signal' as a sequence of either a feature or a target, and denote it as $d^{(t)}_{i,1:t}$. %; it follows that $d_i^{(t)} \in \mathcal{D}^{(t)}, \forall i \in \{1:|\mathcal{D}^{(t)}|\}$.
Thus, at prediction week $t$, the real-time forecasting problem is:
Given $\mathcal{D}^{(t)}_{1:t}$, predict next $k$ values of forecasting target(s), i.e. $\hat{y}_{t+1:t+k}$. Typically for CDC forecasting settings and this paper, our time unit is week, $k=4$ (up to 4 weeks ahead) and our target is COVID-19  mortality incidence (\fdt).


\par\noindent\textbf{Backfill.} %Backfill is present in our data when the following occurs. 
Data revisions (`backfill') are common in real-time forecasting. At prediction week $t+1$, the real-time sequence $\mathcal{D}^{(t+1)}_{1:t+1}$ is available. In addition to the length of the sequences increasing by one (new data point), values of $\mathcal{D}^{(t+1)}_{1:t+1}$ already in $\mathcal{D}^{(t)}_{1:t}$ may be revised i.e., $\mathcal{D}^{(t)}_{1:t} \neq \mathcal{D}^{(t+1)}_{1:t}$. 
% This is equivalent to saying that backfill is present if $\exists t'\in \{1:t\}: d^{(t)}_{i,t'} \neq d^{(t+1)}_{i,t'}$.
Note that previous work has studied backfill limited to $\mathcal{Y}^{(t)}$, while we address it in both $\mathcal{X}^{(t)}$ and $\mathcal{Y}^{(t)}$.



% Therefore, another way to define backfill is: for a given signal $d^{(t)}_{i,1:t}$, backfill is present if $\exists t'\in \{1:t\}: d^{(t)}_{i,t'} \neq d^{(t+1)}_{i,t'}$.  


% second attempt alex
% \par\noindent\textbf{Real time forecasting.} 
% Let $\mathcal{X}_t$ be a set of feature sequences at week $t$ (multi-variate time series) and $\mathcal{Y}_t$ be a set of forecasting label sequence(s) at week $t$.
% Further, we can define our data available at week $t$ as $\mathcal{D}_t = \{ \mathcal{X}_t, \mathcal{Y}_t \}$, which we call \emph{real time sequence}. For clarity in exposition, we refer to signal as a sequence of either a feature or a label, and denoted it as $d_{i,t}$, thus, $d_{i,t} \in \mathcal{D}_t, \forall i \in \{1:|\mathcal{D}_t|\}$.

% Thus, at week $t$, the real time forecasting problem can be simply stated as follows.
% Given $\mathcal{D}_t$, predict the next $k$ values of forecasting label(s), i.e. $\hat{y}_{t+1:t+k}$, 
% where our $k=4$ (4 weeks ahead) and our label is incidence mortality (\fdt).

% \par\noindent\textbf{Backfill.} Backfill is present in our data when the following occurs. At week $t+1$, in addition to the length of the sequences increasing by one, values already in $\mathcal{D}_t$ may be revised. % -- i.e., $d_{i,t}, \ldots, d_{i,o}^{(\infty)}$,
% We can express that by introducing two temporal dimensions to our dataset $\mathcal{D}_t$, \emph{observation week} $o \in \{1:|t\}$ and \emph{revision week} $r \in \{1:|t\}$. 
% $\mathcal{D}_t^{1:t} \neq \mathcal{D}_{t+1}^{1:t}$. We refer to the temporal dimension imposed by the super-index as observation week $o$. As a side note, we want to emphasize that previous work has studied backfill circumscribed to $\mathcal{Y}^{(t)}$, while we address it in both $\mathcal{X}^{(t)}$ and $\mathcal{Y}^{(t)}$.



% harsha
% At week $t$, we are given historical mortality reports (death counts per week) available until week $t$, and we are requested to use this data to make predictions for future weeks. As previously mentioned, the historical data may be subsequently revised by CDC at any week after been released. (count cases reach stability after 2.8 weeks on average).
% Let $Y_i^{(m)}$ represent the official estimate of death counts in week $i$ as per reported/revised at week $m$, where $m>i$. For example, if at week $t$ an estimate for week $t'\leq t$ is released, this will be denoted as $Y_{t'}^{(t)}$, and its future revisions will be denoted with $Y_{t'}^{(t+1)}, Y_{t'}^{(t+2)}, \ldots, Y_{t'}^{(\infty)}$cccc.
% Therefore, the sequence of count cases  given at week $t$ (called \emph{real-time sequence}) is denoted as $ Y^{(t)} = \langle Y_1^{(t)}, Y_2^{(t)}, \ldots, Y_{t}^{(t)} \rangle$, and the \emph{stable sequence} is denoted as $Y^{(\infty)} = \langle Y_1^{(\infty)}, \ldots, Y_{t}^{(\infty)} \rangle$.

% At week $t$, we also refer to $Y_t^{(t)}$ as the \emph{real-time} label or \emph{initial} label. $Y_t^{(\infty)}$ is called the \emph{stable} label.


% Correspondingly, we also look at revisions for exogenous signals used in addition to historical mortality. Let each signal be indexed by an integer $i\in \{1, \dots, K\}$. We denote for a signal indexed by $i\in \{1,2,\dots,K\}$, $F(i)_{t'}^{(t)}$ as the estimate of the signal value for week $t'$ as reported on week $t\geq t'$. Thus the stable sequence for the signal $F(i)^{(\infty)} = \langle F(i)_{1}^{(\infty)}, \dots, F(i)_{t}^{(\infty)} \rangle$.




==> checklist.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See conclusion}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See conclusion}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{We mentioned in folder containing code}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{Added \dtst dataset in supplementary}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> dump.tex <==
\onecolumn
\title{Supplementary}
\appendix

\section{Appendix}

Optionally include extra information (complete proofs, additional experiments and plots) in the appendix.
This section will often be part of the supplemental material.







\section{Nature of backfill dynamics (more details)}

\subsection{Notation considering Delay}
\alex{TODO: add delay to notation}

In this section, we study important properties of the revision dynamics of our signals. We introduce some concepts and definitions to aid in understanding of our empirical observations and method.

%Here we give the background, notation and definitions to set up backfill in real-time forecasting. 
%In addition, it is important to note that the data in backfill is the same used for real-time forecasting, but seen from a different perspective.

% first attempt alex
% \aditya{I do not understand the 'real-time sequence'. is $D^t$ for a particular 't' the sequence? How can one timestamped dataset be a sequence. We need to say what is Xt and Yt, maybe Xti is a time-series from [1..t] something like that}
\par\noindent\textbf{Real-time forecasting.} 
At prediction week $t$, $x^{(t)}_{i,1:t}$ is a time series from 1 to $t$ for feature $i$, and the set of all features results in the multi-variate time series $\mathcal{X}^{(t)}_{1:t}$\footnote{In practice, delays are possible too, i.e, at week $t$, we have data for some feature $i$ only until $t-\delta_i$. All our results incorporate these situations. We defer the minor needed notational extensions to supplement for clarity.}.
Similarly, $\mathcal{Y}^{(t)}_{1:t}$ is the forecasting label(s) time series.
Further, let's call all data available at time $t$, $\mathcal{D}^{(t)}_{1:t} = \{ \mathcal{X}^{(t)}_{1:t},  \mathcal{Y}^{(t)}_{1:t} \}$ as \emph{\underline{real-time sequence}}. 
%to our data available at time $t$ and denote it as $\mathcal{D}^{(t)}_{1:t} = \{ \mathcal{X}^{(t)}_{1:t}, \mathcal{Y}^{(t)}_{1:t} \}$. 
For clarity we refer to `signal' as a sequence of either a feature or a label, and denote it as $d^{(t)}_{i,1:t}$. %; it follows that $d_i^{(t)} \in \mathcal{D}^{(t)}, \forall i \in \{1:|\mathcal{D}^{(t)}|\}$.
Thus, at prediction week $t$, the real-time forecasting problem is:
\emph{Given $\mathcal{D}^{(t)}_{1:t}$, predict next $k$ values of forecasting label(s), i.e. $\hat{y}_{t+1:t+k}$}. Typically for CDC forecasting settings and this paper, our time unit is week, $k=4$ (up to 4 weeks ahead) and our label is COVID-19  mortality incidence (\fdt).


\par\noindent\textbf{Revisions.} %Backfill is present in our data when the following occurs. 
Data revisions (`backfill') are common. At prediction week $t+1$, the real-time sequence $\mathcal{D}^{(t+1)}_{1:t+1}$ is available. In addition to the length of the sequences increasing by one (new data point), values of $\mathcal{D}^{(t+1)}_{1:t+1}$ already in $\mathcal{D}^{(t)}_{1:t}$ may be revised i.e., $\mathcal{D}^{(t)}_{1:t} \neq \mathcal{D}^{(t+1)}_{1:t}$. 
% This is equivalent to saying that backfill is present if $\exists t'\in \{1:t\}: d^{(t)}_{i,t'} \neq d^{(t+1)}_{i,t'}$.
Note that previous work has studied backfill limited to $\mathcal{Y}^{(t)}$, while we address it in both $\mathcal{X}^{(t)}$ and $\mathcal{Y}^{(t)}$.
It is important to note that the data in backfill is the same used for real-time forecasting, but seen from a different perspective.

% \par\noindent\textbf{Backfill temporal dimension.} 
\par\noindent\textbf{Backfill sequences:} 
Another useful way to look at backfill is by focusing on revisions of a single value. Let's focus on the value of signal $i$ at an \emph{\underline{observation week}} $t'$. 
%This $t'$ is also the week of initial release, i.e. the week the value of signal $i$ for $t'$ was first reported.
For this observation week, the value of the signal can be revised for any $t>t'$ which induces a sequence of revisions.
% for any $i$.
We refer to \emph{\underline{revision week}} $r\geq0$ as the relative amount of time that has passed since the observation week $t'$. %, consequently, its domain is $r=\{0:t\}$.

% The observation week may coincide with the week of its initial released, but in practice it is common to see delays, especially in traditional surveillance signals because of the time required for processing clinical information~\cite{yang2015accurate}.

\begin{defn}
(Backfill Sequence \bseq) For signal $i$ and observation week $t'$, its backfill sequence is $\bseq(i,t')= \langle d_{i,t'}^{(t')}, d_{i,t'}^{(t'+1)}, \ldots, d_{i,t'}^{(\infty)} \rangle$, where $d_{i,t'}^{(t')}$ is the \emph{\underline{initial value}} of the signal and $d_{i,t'}^{(\infty)}$ is the \emph{\underline{stable value}} of the signal.
\end{defn}
\begin{defn}
(Backfill Error \be) For revision week $r$ of a backfill sequence, the backfill error is
 $  \be(r) = | d^{(t'+r)}_{i,t'} - d^{(\infty)}_{i,t'}|~/~|d^{(\infty)}_{i,t'}|.$
\end{defn}
\begin{defn}
(Stability time \bd) of a backfill sequence \bseq is the revision week $r^*$ that corresponds the minimum $r$ for which the backfill error \be is less than $\epsilon$ for all $r>r^*$, i.e., the time when \bseq converges. % asymptotically stabilizes. 
\end{defn}
\textit{Note:}  
% Intuitively, this is a sequence describing the revision evolution of a signal value since its initial release.
Since it is infeasible to estimate $d^{(\infty)}_{i,t'}$, we use the last value of the \bseq.
We found that in our dataset everything stabilizes after 20, and the length of our backfill sequences is at least 7.
In the case our \bseq does not have $\be<\epsilon$, we assume \bd is the length of \bseq.
% we approximate it with $d^{(t'+T)}_{i,t'}$ where $T=\min(20, T_a)$ and $T_a$ is the last available revision week (as mentioned before, $T_a\geq7$).
% \emph{Note:} Again, in practice, we assume all values are stabilized by week $T$ worst case. 




\subsection{Backfill statistics}
We first study different facets of the significance of backfill in \dtst.
Using our definitions, we generate a backfill sequence for every combination of signal, observation week, and region (not all signals are available for all regions). In total, we generate \emph{more than} $40,000$ backfill sequences.

%\alex{note that we did not introduce region before, so we are being a bit careful when saying that we aggregate over it -- does it look good?}
\paragraph{Backfill error \be is significant}
We analyze the significance of the backfill error in the \dtst dataset by looking at the largest values of backfill error, which are for the initial values (i.e., $\be(r=0)$, but for simplicity we refer to it as $\be$). 
We average \be of each signal over all observation weeks and all regions (states and national). 
Figure~\ref{fig:obs1} shows the average \be of each feature type. Note that some signals exhibit very high \be such as \frec which averages around 81.1. In contrast \fvnt and \ficu show very low \be of 0.001 and 0.014. 
% \alex{I recommend to make clear here that even digital indicators also suffer from backfill, which is something that nobody has pointed out before as people has focused on traditional surveillance data}
In addition, it is well known that traditional surveillance data suffers from backfill~\cite{yang2015accurate}, however, past work has not pointed out that digital indicators -- such as mobility, exposure and social surveys -- while more readily available, they also suffer from backfill. We found that these the signals on these three groups have a \be of XX.

\begin{obs} (Significance of \be across signals)
% The median \be of all signals, each of which is averaged over all regions, is 0.32;
The median average \be per signal (averaged over all regions) is 0.32;
therefore, initial values are often corrected in 32\% on each signal.
\label{obs:obs1}
\end{obs}


% \begin{figure}[h]
%     \centering
%     \begin{minipage}{.49\textwidth}
%     \centering
%     \begin{subfigure}{.49\linewidth}
%     \centering
%     \includegraphics[width=.95\linewidth]{Images/Obs1a.pdf}
%     \caption{Average \be for each signal type}
%     \label{fig:obs1}
%     \end{subfigure}
%     \begin{subfigure}{.49\linewidth}
%     \centering
%     \includegraphics[width=.95\linewidth]{Images/stime.png}
%     \caption{Average \be for each region}
%     \label{fig:obs1_1}
%     \end{subfigure}
%     \caption{Most signals have significant \be. Average \be across regions and features is not uniform and varies widely}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{.49\textwidth}
%     \centering
%     \begin{subfigure}{.49\linewidth}
%     \centering
%     \includegraphics[width=.95\linewidth]{Images/Obs2a.pdf}
%     \caption{Average \bd for each signal type}
%     \label{fig:obs2}
%     \end{subfigure}
%     \begin{subfigure}{.49\linewidth}
%     \centering
%     \includegraphics[width=.95\linewidth]{Images/berr.png}
%     \caption{Average \bd for each region}
%     \label{fig:obs2_2}
%     \end{subfigure}
%     \caption{\bd varies across signals and across regions \alex{fix y label to \bd}}
%     \end{minipage}
% \end{figure}

There is also a significant variation of \be across regions. As seen in Figure~\ref{fig:obs1_1}, states like NY and NJ show the highest average \be, which are 25.16 and 21.57, respectively. This is largely due to the fact that \be of \frec is 521.3 and 444.3 in average for NY and NJ, respectively.
In contrast, states like FL, CA, IL, WA and GA show lower \be, which averages around 0.384, and the \frec \be for these regions is zero.

\begin{obs} (Significance of \be across regions)
% The median of set of average \be of all regions (averaged over all signals) is 2.8
The median average \be per region (averaged over all signals) is 2.8; therefore, initial values are often corrected in 280\% on each region.
\label{obs:obs2}
\end{obs}


\paragraph{Stability time \bd is significant}

Next we study the stability time \bd of our \dtst.  Average \bd for each signal type is shown in Figure~\ref{fig:obs2}. We observed that \fcvn stands out by taking about 16.4 weeks to fully stabilize. The average \bd of a region also varies widely (see Figure~\ref{fig:obs2_2}) from 1.55 weeks for GA to 3.83 weeks for TX. We also have to ideally wait for 2.8 weeks to receive stable ground truth to evaluate different models' actual accuracy which may be prohibitive for real-time model evaluation and decision making.

\begin{obs} (\bd of features and label)
% \begin{obs} (\bd of stable labels)
% Average \bd of ground truth labels (\fdt) is 2.8 weeks.
Average \bd (across all regions) of our features in \dtst is 3.82 weeks and in our label \fdt  is 2.8 weeks.
\end{obs}


\subsection{Backfill sequence \bseq patterns}
\label{subsec:patterns}
Next we look at \bseq of signals over all regions in \dtst to identify interesting patterns.

\paragraph{Canonical \bseq behaviors}

We observed that the \bseq patterns are of wide variety. We clustered them to find canonical behaviors. In order to derive these clusters, we performed K-means clustering over all the \bseq of \dtst using Dynamic Time Warping (DTW) as the distance metric between these time series. The reason we used DTW is two fold: a) it enables us to compare time series of different magnitudes. This is important because of the large variation in magnitudes of across times, signals and regions. b) DTW also allows us to measure similarities between two $\bseq$s of different lengths.

\begin{obs} (\bseq clusters)
Five canonical behaviors were observed through clustering all \bseq of \dtst.
\label{obs:obs3}
\end{obs}

The behaviors of these clusters as shown in Figure \ref{fig:patterns} can be described as:
\begin{enumerate*}
    \item \textbf{Early decline} (\bed): \bseq values stabilizes quickly (within a week) to a lower stable value.
    \item \textbf{Early increase} (\beinc): \bseq values increase in 2 to 5 weeks and stabilize.
    \item \textbf{Steady/spike} (\bst): \bseq values either remain constant (no significant revision) or due to reporting errors there may be anomalous values in between. (E.g., for a particular week in middle of \bseq the signals are revised to 0 due to reporting error).
    \item \textbf{Late increase} (\blin): \bseq values increase and stabilize very late during revision.
    \item \textbf{Mid decrease} (\bmd): \bseq values change and stabilize after 8 to 10 weeks of revision.
\end{enumerate*}

Most \bseq broadly follow one of the canonical behaviors listed above though there can be smaller complex deviations.
\bed and \beinc indicate lower \bd whereas \blin and \bmd indicate higher \bd. 
We found that 94\% of mobility features, 96.2\% of exposure features and 93.1\% for Social Survey fall in \bed and \beinc where as the number falls to 42\%, 37\% for line list features. The rest of \bseq are mostly found in \blin and \bmd. We see that digital features types (mobility and exposure), which are expected to be reported accurately in real-time also undergo revision in some instances.
%\alex{here or in the prev observation, say that digital indicators are quicker in stabilizing, which makes sense, however, in some cases they can take longer times; therefore, it makes sense to also include them in our approach}
Only 6.4\% of \bseq fall under \bst cluster which consists of \bseq with negligible revisions.
%We found that over 83\% of \bseq s fall in cluster 1 or 2. 
%One would expect that there would be large similarity between in either signal index or regions of curves in a cluster. 
We also observed that no cluster showed large proportion from a single signal or region with only single exception in \bed, which mostly consists of \bseq from \frec.

\begin{obs} (Regional Variety in \bseq clusters)
No cluster has over 21\% of \bseq from the same region.
\label{obs:obs4}
\end{obs}

\begin{obs} (Signal variety in \bseq clusters)
No cluster (except \bed) has over 36\% of \bseq from the same signal.
\label{obs:obs5}
\end{obs}
Leveraging these similarities in revisions signals can be useful for predicting \emph{stable} labels. 

\subsection{Model bias}
Next we look at how \be influence training and evaluation of models.
We analyze the top performing real-time forecasting models as per the comprehensive evaluation of all models in the \hub~\cite{cramer2021evaluation}. YYG-ParamSearch (\yyg) and UMass-MechBayes (\umass) are mechanistic models and CMU-TimeSeries (\cmu) and GT-DeepCOVID (\deepcovid) are statistical models. The \hub ensemble (\ensemble) is composed from all contributing models to the hub and it is the top performing one.


% \begin{figure}[h]
%     \centering
%     \begin{subfigure}{.19\linewidth}
%     \includegraphics[width=.9\linewidth]{Images/Ensemble.pdf}
%     \caption{\ensemble} % CovidHub-Ensemble
%     \end{subfigure}
%     \begin{subfigure}{.19\linewidth}
%     \includegraphics[width=.9\linewidth]{Images/GTDC.pdf}
%     \caption{\deepcovid} % DeepCovid
%     \end{subfigure}
%      \begin{subfigure}{.19\linewidth}
%     \includegraphics[width=.9\linewidth]{Images/YYG.pdf}
%     \caption{\yyg} % YYG-ParamSearch
%     \end{subfigure}
%     \begin{subfigure}{.19\linewidth}
%     \includegraphics[width=.9\linewidth]{Images/Umass.pdf}
%     \caption{\umass} %UMass-MechBayes
%     \end{subfigure}
%     \begin{subfigure}{.19\linewidth}
%     \includegraphics[width=.9\linewidth]{Images/CMU.pdf}
%     \caption{\cmu} % CMU-TimeSeries
%     \end{subfigure}
%     \caption{Relationship between \be and \revmae for top 5 \hub models \harsha{Will work on fonts}}
%     \label{fig:obs_corr}
% \end{figure}


\begin{wraptable}{r}{0.26\linewidth}
\vspace{-0.2in}
\begin{tabular}{|l|l|}
\hline
\textbf{Model}    & \textbf{PCC} \\ \hline
\ensemble & -0.327       \\ \hline
\deepcovid      & -0.322       \\ \hline
\yyg   & 0.110        \\ \hline
\umass   & -0.291       \\ \hline
\cmu    & -0.468       \\ \hline
\end{tabular}
\caption{Pearson Correlation Coefficient (PCC) between \be and \revmae using stable labels over real-time labels}
\label{tab:pcc}
\vspace{-0.26in}
\end{wraptable}

\paragraph{Dependence of \be on performance}
It is expected that a well trained statistical model on real-time signals will perform worse as the \be on the labels increase. However, 
%due to complex \bseq patterns and each model leveraging \dtst differently, 
we found that models  differ in how their performance is impacted by \be on the label. To study this relationship, we observe the relationship between \be and reduction in MAE on using \emph{stable} labels for evaluation over \emph{real-time} labels. We denote this decrease in MAE for model $M$'s prediction at week $t$ for region $r$ as $\revmae(M,t,r)$.


We show the relationship between \be and \revmae for each of top models of \hub in Figure \ref{fig:obs_corr}.
\ensemble, \deepcovid and \umass have similar plots whereas \yyg and \cmu show different behavior. We also compute the Pearson correlation coefficient (PCC) between \be and \revmae for each model to look at average correlation of performance change with \be in Table \ref{tab:pcc}. Interestingly, we observe that for \yyg, PCC is positive, indicating that \yyg's scores are actually due to larger \be on labels. We also see significant differences in PCC for \yyg and \cmu in over other models.
 
\begin{obs} (Correlation between \be and \revmae)
Pearson correlation between \be and \revmae is negative for some models while positive for others; therefore, there is an underlying non-linear relationship between backfill and model's performance.
\label{obs:obs6}
\end{obs}






\paragraph{Detriment of using real-time labels to measure of model accuracy}


In order to evaluate forecasting models to report an accurate estimate of future \cvnt mortality, model evaluators rely upon the accuracy of the model with respect to \emph{real-time} labels. Since these labels undergo revisions (about 5\% on average) evaluation metrics are not the true indicators of model's performance.

% \begin{wrapfigure}{r}{.5\linewidth}
%     \vspace{-0.23in}
%     \centering
%     \begin{subfigure}{.4\linewidth}
%     \centering
%     \includegraphics[width=.9\linewidth]{Images/MAE.pdf}
%     \caption{MAE scores}
%     \label{fig:obs4_mae}
%     \end{subfigure}\hspace{0em}%
%     \begin{subfigure}{.4\linewidth}
%     \centering
%     \includegraphics[width=.9\linewidth]{Images/MAPE.pdf}
%     \caption{MAPE scores}
%     \label{fig:obs4_mape}
%     \end{subfigure}
%     \vspace{-0.1in}
%     \caption{Relation of performance metrics (MAE, MAPE) for real-time and stable labels vary significantly causing evaluators to over-estimate the accuracy of the models.}
%     \label{fig:obs4}
%     \vspace{-0.3in}
% \end{wrapfigure}

We show the relation between real-time measured scores and scores measured with revised labels in Figure \ref{fig:obs4}. We see that the scores are not similar with real-time scores over estimating model accuracy. The average difference in scores is positive (real-time MAE and MAPE is lower than stable MAE and MAPE) which implies that evaluators overestimate the performance of the models' forecasting ability.

\begin{obs}
MAE and MAPE evaluated at real-time overestimates model performance by 2.69\% and 6.9\% on average, respectively.
\label{obs:obs7}
\end{obs}

